Step-Calibrated Diffusion for Biomedical Optical Image Restoration

High-quality, high-resolution medical imaging is essential for clinical care. Raman-based biomedical optical imaging uses non-ionizing infrared radiation to evaluate human tissues in real time and is used for early cancer detection, brain tumor diagnosis, and intraoperative tissue analysis. Unfortunately, optical imaging is vulnerable to image degradation due to laser scattering and absorption, which can result in diagnostic errors and misguided treatment. Restoration of optical images is a challenging computer vision task because the sources of image degradation are multi-factorial, stochastic, and tissue-dependent, preventing a straightforward method to obtain paired low-quality/high-quality data. Here, we present Restorative Step-Calibrated Diffusion (RSCD), an unpaired diffusion-based image restoration method that uses a step calibrator model to dynamically determine the number of steps required to complete the reverse diffusion process for image restoration. RSCD outperforms other widely used unpaired image restoration methods on both image quality and perceptual evaluation metrics for restoring optical images. Medical imaging experts consistently prefer images restored using RSCD in blinded comparison experiments and report minimal to no hallucinations. Finally, we show that RSCD improves performance on downstream clinical imaging tasks, including automated brain tumor diagnosis and deep tissue imaging. Our code is available at https://github.com/MLNeurosurg/restorative_step-calibrated_diffusion.

==> 20_Reproducibility_Checklist.tex <==
\section{Reproducibility Checklist}

Unless specified otherwise, please answer “yes” to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled “Reproducibility Checklist” at the end of the technical appendix.

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \textbf{(yes), see Algorithm 1}

\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \textbf{(yes)}

\item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper \textbf{(yes)}

\item Does this paper make theoretical contributions? \textbf{(no)}

\item Does this paper rely on one or more datasets? \textbf{(yes)}

\item A motivation is given for why the experiments are conducted on the selected datasets \textbf{(yes)}

\item All novel datasets introduced in this paper are included in a data appendix. \textbf{(NA)}

\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{(NA)}

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{(yes)}

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{(yes)}

\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. \textbf{(yes), see Appendix~\ref{app:near}}

\item Does this paper include computational experiments? \textbf{(yes)}

\item Any code required for pre-processing data is included in the appendix. \textbf{(yes)}

\item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{(yes)}

\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{(yes)}

\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \textbf{(yes)}

\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{(yes)}

\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{(yes), see Appendix~\ref{app:compres}}

\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{(yes), see Experiments Section}

\item This paper states the number of algorithm runs used to compute each reported result. \textbf{(yes), see Appendix~\ref{app:experiments}}

\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{(yes), the perceptual metrics (like FID and CMMD) are distributional in nature.}

\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{(no)}

\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{(yes), see Table~\ref{tab:hyperparameter} in Appendix~\ref{app:hyperparameter}}

\item This paper states the number and range of values tried per (hyper-) parameter during the development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{(yes), see Appendix~\ref{app:hyperparameter}}


\end{itemize}
